Exploring the Limits of Static Failover Routing

We present and study the Static-Routing-Resiliency problem, motivated by routing on the Internet: Given a graph $G$, a unique destination vertex $d$, and an integer constant $c>0$, does there exist a static and destination-based routing scheme such that the correct delivery of packets from any source $s$ to the destination $d$ is guaranteed so long as (1) no more than $c$ edges fail and (2) there exists a physical path from $s$ to $d$? We embark upon a systematic exploration of this fundamental question in a variety of models (deterministic routing, randomized routing, with packet-duplication, with packet-header-rewriting) and present both positive and negative results that relate the edge-connectivity of a graph, i.e., the minimum number of edges whose deletion partitions $G$, to its resiliency.

==> results.tex <==
\section{List of results}

\vspace{2mm}
\rephrase{Theorem}{\ref{theo:vertex-connectivity-impossibility}}{
 \vertexConnectivityTheorem
}
\vspace{2mm}


\vspace{2mm}
\rephrase{Theorem}{\ref{theo:no-circular-ordering}}{
 \noCircularOrdering 
}
\vspace{2mm}

\vspace{0.5mm}

\rephrase{Theorem}{\ref{theo:no-k-resiliency}}{
 \noKResiliency 
}
\vspace{1.5mm}

\vspace{0.5mm}
\rephrase{Theorem}{\ref{theo:2-resiliency}}{
 \TwoResiliency 
}
\vspace{1.5mm}

\newcommand{\HypercubeResiliency}{For any $d$-dimensional hypercube graph $G$ there exists a routing  of $G$ that is $(d-1)$-resilient.}

\begin{theorem}\label{theo:hypercube-resiliency}
\HypercubeResiliency
\end{theorem}

\vspace{2mm}
\rephrase{Theorem}{\ref{theo:generalized-hypercube-resiliency}}{
 \GeneralizedHypercubeResiliency
}
\vspace{2mm}


\vspace{2mm}
\rephrase{Theorem}{\ref{theo:grid-resiliency}}{
 \GridResiliency
}
\vspace{2mm}


\vspace{2mm}
\rephrase{Theorem}{\ref{theo:clos-resiliency}}{
 \ClosResiliency
}
\vspace{2mm}


\vspace{2mm}
\rephrase{Theorem}{\ref{theo:chordal-resiliency}}{
 \ChordalResiliency
}
\vspace{2mm}








\subsection{List of results with proofs}

We say that a routing function at vertex $v$ is a {\em circular ordering routing function} if 
it can be constructed from an ordered circular sequence $N=(n_1,\dots,n_l)$ of the neighbors of $v$
by setting $f^v(n_i,A)=n^*$, where $A$ is a set of neighbors of $v$ no longer directly reachable from $v$ and 
$n^*$ is the first vertex not in $A$ that follows $n_i$ in $N$.
Intuitively, $v$ forwards a packet received from $n_i$ to $n_{i+1}$, unless $(n_i,n_{i+1})$ has failed. 
In that case, it tries to forward to $n_{i+2}$, and so on. 
If each vertex implements a circular ordering routing function we say that routing is a
{\em circular ordering routing}.


\vspace{2mm}
\rephrase{Theorem}{\ref{theo:no-circular-ordering}}{
 \noCircularOrdering 
}
\vspace{2mm}

\begin{proof}
 \begin{figure}[tb]
  \centering
    \includegraphics[width=.7\columnwidth]{figures/candidate-counterexample}
    \caption{ An instance that don't admit any circular ordering routing that is $2$-resilient. Vertex $d$
    is the destination vertex. }
\label{fig:candidate-counterexample-ordering}
\end{figure}
We prove that the graph $G$ depicted in Figure~\ref{fig:candidate-counterexample-ordering},
which is $3$-connected, does not admit any circular ordering routing scheme. Vertex $d$ is the destination. 
Suppose, by contradiction, that there exists a circular ordering routing of $G$. 
Since the instance is symmetric, w.l.o.g, assume that $o$ routes clockwise, i.e., a 
packet from $x$ is sent to $z$, from $z$ to $y$, and from $y$ to $x$. 
W.l.o.g, assume that $o$ sends its first packet $p$ to $y$ when none of its incident edges has failed. 

We first claim that vertices $y$, $a$, and $z$ route counterclockwise. 
Suppose, by contradiction, that (i) $y$ routes clockwise, or (ii) 
$a$ routes clockwise, or (iii) $z$ routes clockwise.
In case (i), if both edges $(a,d)$ and $(z,a)$ failed, $p$ is routed 
through $(y,a,z,o)$. In turn, since $o$ routes clockwise, it forwards $p$ to $y$ 
and a forwarding loop arises, which is a contradiction. Case (ii) and (iii) are similar to case (i), but different
edges fail.
In case (ii), if both edges $(y,b)$ and $(z,a)$ fail, $p$ is routed 
through $(y,a,z,o)$ and a forwarding loop arises, which is a contradiction. 
In case (iii), if both edges $(y,b)$ and $(a,d)$ fail, $p$ is routed 
through $(y,a,z,o)$ and a forwarding loop arises, which is a contradiction.

Observe that if $c$ sends a packet $p$ to $x$, if $x$ routes clockwise it forwards it directly to $b$, 
otherwise, if $x$ routes counterclockwise, $p$ is forwarded
through $o$, $z$, $a$, $y$, $o$, $x$, and, also in this case, to $b$. 
Consider the scenario where both edges $(c,d)$ and $(b,d)$ failed. A packet $p$ sent from $o$
to $y$ will be routed through $y$, $c$, and $b$. By the previous observation, $p$
will be routed to $b$ and will continue through $z$, $o$, and again to $y$. Hence, 
a forwarding loop arises also in this case, which is a contradiction.
\end{proof}

One may argue that in the previous proof, when $a$ receives a packet, it does not
forward it directly to $d$ even if it has a direct connection to $d$. It is possible
to prove that circular ordering routing cannot achieve $(k-1)$-resiliency even if neighbors
of $d$ are allowed to violate the circular ordering routing constraints.

\vspace{2mm}
\rephrase{Theorem}{\ref{theo:vertex-connectivity-impossibility}}{
 \vertexConnectivityTheorem
}
\vspace{2mm}

\begin{proof}
 Consider the graph $G$ used in the proof of Theorem~\ref{theo:no-circular-ordering} in Figure~\ref{fig:candidate-counterexample-ordering}. 
Replace each edge of $G$ that is (not) incident to $d$ with a path consisting of three (two) edges. 
We call the added vertices \emph{intermediate} vertices and the old ones \emph{original} vertices.
See Figure~\ref{fig:candidate-counterexample-ordering-3edges}.
\begin{figure}[tb]
  \centering
    \includegraphics[width=.7\columnwidth]{figures/candidate-counterexample-3edges}
    \caption{ An instance such that, for any routing scheme, a forwarding loop may arise when $o$
    sends a packet even if only two vertex failure happen. Small black circles represent vertices. 
    W.r.t. Figure~\ref{fig:candidate-counterexample-ordering}, a link failure $(x,y)$ is 
    modelled as the failure of any inner black vertex that connects $x$ and $y$.}
\label{fig:candidate-counterexample-ordering-3edges}
\end{figure}
Each original vertex of $G$ remains $3$-connected to the destination $d$. 
We now show that 
the original $8$ vertices, but $d$,  must implement a circular ordering routing function, 
otherwise a routing loop may arise. By Theorem~\ref{theo:no-circular-ordering}, this is not 
possible, hence a contradiction.

Routing functions at intermediate vertices are trivial. A packet is never bounced back unless an incident link failed. 
Hence, we only compute routing functions at original vertices. 
We will consider only failures between intermediate vertices,
thus a routing scheme for each original vertex is just a table with three entries: Where to send a packet arrived through each of the three links.
Hence, we simplify our routing function notation as follows. Let $f^v(n)=n'$ be a routing
function at vertex $v$ such that a packet received from $n \in \{N(v) \cup \emptyset\}$ is 
forwarded to $n' \in N(v)$, where $\emptyset$ represents the fact that a packet is originated at
$v$. 

First, for each vertex $v$ we have that $f^v(n) \ne n$, where $n \in N(v)$, i.e. no vertex bounces a 
packet back to the link where it received it. In fact, in case that link had a 
dead-end ahead created by a link failure between two intermediate vertices, this packet will be trapped in a loop 
between $n$ and $v$. 

Second, all entries in the routing table are distinct. Otherwise, suppose by contradiction that 
$f^v(n_1) = f^v(n_2) = n_3$, where $n_1,n_2,n_3 \in N(v)$. W.l.o.g., assume that $f^v(n_3)=n_1$.
If both $n_1$ and $n_3$ are only connected to $v$ because of two link failures, 
then a packet will loop among $n_3$, $v$, and $n_1$. Hence, original vertices must use a circular
ordering routing scheme. However, we proved above that there does not exist
any circular ordering routing scheme for the simplified graph, which means that we cannot
compute a vertex-connectivity-resilient routing scheme for this graph. 
\end{proof}


\vspace{0.5mm}

\rephrase{Theorem}{\ref{theo:no-k-resiliency}}{
 \noKResiliency 
}
\vspace{1.5mm}

\begin{proof}
 We show a $2$-connected graph that does not admit any $2$-resilient routing scheme (see Fig.~\ref{fig:graph1}). 
% There are many graphs with such property, but presented is one of the smallest. 
% In this section we prove that no static routing scheme can be 1-connectivity-resilient.

The destination is the vertex $1$ \notemarco{we must change these pictures and write $d$}. The vertices $2$, $3$, $4$, and $5$ all have $3$ links with other vertices.
 Small dots on the picture are intermediate vertices. 
% They are needed to simplify the proof. 
As in the proof of Theorem~\ref{theo:vertex-connectivity-impossibility}, we consider only 
failures between intermediate vertices. This implies that (i) for each vertex $v$ 
we have that $f^v(n) \ne n$, where $n \in N(v)$, i.e. no vertex bounces a 
packet back to the link where it was received, and (ii) all entries in the routing table are distinct.
% 
Therefore, each of the four key vertices, i.e., $2$, $3$, $4$, and $5$, must implement
a circular ordering routing function. There are only two cyclic permutations 
for $3$ elements, i.e., a clockwise or counterclockwise ordering of the neighbors.

First, we will consider vertices $3$ and $5$. Two cases are possible: either (i) vertices $3$ and $5$ 
have circular ordering functions with different orientations, or (ii) not.
% There are $4$ routing schemes for these two vertices. Anyway, because of the symmetry of the graph,
% there are only $2$ distinct possible scenarios. In the first one, vertices $3$ and $5$ have same
% the same clockwise order of edges. 
% In the first case, by symmetry of the graph, w.l.o.g., assume that the order is clockwise. 
% In the second routing they have different orders of edges.
In the first case, by symmetry of the graph and w.l.o.g., assume that $3$ routes clockwise and
$5$ counterclockwise. Then, if two link failures are sufficient to create a forwarding loop
for packets originating on the first intermediate vertex between vertices $3$ and $2$, as 
shown in Fig.~\ref{fig:graph2} .
That packet visits vertex $3$. After that, it is routed 
towards vertex $4$ and, consequently, regardless of ordering at vertex $4$, it goes 
to vertex $5$, where it is routed back to vertex $3$. From vertex $3$, it is routed 
toward vertex $2$, therefore, creating a loop.

In case (ii), by symmetry of the graph and w.l.o.g., assume that both $3$ and $5$ route
clockwise.
There are $4$ routing schemes for different ordering at vertices $2$ and $4$. All these
possibilities are analyzed case-by-case and are shown from Fig.~\ref{fig:graph3} to Fig.~\ref{fig:graph4a}.
%  
% Therefore, we have shown that there are no static routing scheme which will be 2-resilient.
% Note, that given proof assumes there may be up to two simultaneous link failures 
% to argue that routing at each vertex should be in a round manner. Thus it does not 
% contradict with existence of 1-resilient routing scheme for any graph.
% 
\begin{figure}[t]
% \centering
\begin{minipage}[t]{0.4\columnwidth}%
% \vspace{0.3in}
\includegraphics[]{figures/graph1.pdf}
\caption{Graph.}\label{fig:graph1}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[]{figures/graph2.pdf}
\caption{Regardless of ordering at vertex $4$ there is a loop starting near vertex $3$.}\label{fig:graph2}
\end{minipage}
\begin{minipage}[t]{0.4\columnwidth}%
% \vspace{0.3in}
\includegraphics[]{figures/graph3.pdf}
\caption{Packet will loop if it starts on path between vertices $5$ and $3$ regardless of its direction}\label{fig:graph3}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[]{figures/graph3a.pdf}
\caption{Packet starting near vertex $4$ will always loop.}\label{fig:graph3a}
\end{minipage}
\begin{minipage}[t]{0.4\columnwidth}%
% \vspace{0.3in}
\includegraphics[]{figures/graph4.pdf}
\caption{Loop starts near vertex $2$}\label{fig:graph4}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.4\columnwidth}%
\includegraphics[]{figures/graph4a.pdf}
\caption{Loop starts near vertex $4$.}\label{fig:graph4a}
\end{minipage}
\end{figure}
\end{proof}



\vspace{0.5mm}
\rephrase{Theorem}{\ref{theo:2-resiliency}}{
 \TwoResiliency 
}
\vspace{1.5mm}

\begin{proof}
A set of directed spanning trees is \emph{arc-disjoint} if for any pair of them, they do not 
have any directed edge in common.
We use the term \emph{arc} and directed edge interchangeably.
Gopalan and Ramasubramanian~\cite{three-trees} showed that there exist $k$ \emph{arc-disjoint}
directed spanning trees rooted at $d$ for any $k$-connected graph, i.e., each tree does not have any arc in common.
Figure~\ref{fig:tetraider} shows an example of a $3$-connected graph 
with $3$ arc-disjoint trees.


\begin{figure}[ht]
 \begin{center}
 \includegraphics[width=.5\columnwidth]{figures/tetraider.pdf}
 \caption{A 3-connected graph with marked three arc-disjoint trees rooted at the top vertex.}
 \label{fig:tetraider}
 \end{center}
\end{figure}

We can utilize these trees to construct a $2$-resilient routing scheme. Let us call these trees Blue, Red and Green. 
We propose two different techniques. 
In the first one, all vertices use the same spanning trees in
the absence of link failures. A packet is guaranteed to reroute on another spanning tree at most twice (assuming only two link failures).
In the second one, each vertex can randomly pick the color of the first spanning
tree to be used. This allows each vertex to choose the shortest path to the destination, which, in the absence of failure,
leads to a better network utilization of the network. However, in the presence of two link failures, a packet may be rerouted
to another spanning tree four times. We present both techniques.
% Consider we already constructed trees. 
% Therefore, each directed link may be colored red, blue or black color (or be uncolored).
Observe that each vertex has an outgoing link of each color.

\vspace{.1in}
\noindent\textbf{Technique 1. } 
When a vertex different from the destination vertex must route a packet $p$, it performs the following actions :
\begin{enumerate}
\item If a vertex originates $p$, it forwards it through the Red outgoing link.
\item If the outgoing link of the same color of the ingoing link has not failed, it forwards $p$ through that link (i.e., no color change).
\item If the ingoing link is Red and the outgoing Red link has failed, then forward $p$ through 
the outgoing link of the same color $c$ of the reversed outgoing Red link. If that link failed, use the third remaining color (neither Red nor
$c$). If  the reversed link is uncolored, then forward $p$ through any of the remaining two trees.
\item If the ingoing link is Blue or Green and the outgoing link of the same color had failed:
use the third remaining color (neither Red nor the color of the ingoing link).
\end{enumerate}
The decisions are made only based on the inbound link and set of failed adjacent links. Therefore it is a static routing.
Such routing will always guide a packet to the destination $d$ for any 2 links failures.


We now show that this routing scheme is $2$-resilient. 
A packet $p$ is routed along the Red tree as long as it encounters a failure. 
It may reach destination just using a Red tree, or encounter a failed link somewhere along the Red branch of the tree.
Let us denote the failed link as $e$.
W.l.o.g., assume that the reversed edge of $e$ is colored Blue.
From now on, the packet will use the Blue tree. It may reach a destination or encounter a failed link $e'$.
Since a tree does not have a cycle, $e'$ is a different link w.r.t. $e$. 
From now on, $p$ is routed along the Green tree. Since a tree does not have a cycle, $p$ cannot encounter $e'$ anymore.
Because link $e$ is colored in Red and Blue, $p$ will not be forwarded on it while it is routed along the Green tree. 
Therefore, $p$ is guaranteed to reach the destination.
If while using the Red tree a packet encounters two failed outgoing links, 
it can use the third colored outgoing link. Because there are no cycles, the remaining path will not traverse any of the two failed links.

\vspace{.1in}
\noindent\textbf{Technique 2. }
We first compute a random circular ordering $<c_0,c_1,c_2>$ of the spanning trees (e.g., $<\text{Blue},\text{Red},\text{Green}>$).
When a vertex different from the destination vertex must route a packet $p$, it performs the following actions :
\begin{enumerate}
\item If a vertex originates $p$, it forwards it on an arbitrary spanning tree.
\item If the outgoing link of the same color of the ingoing link has not failed, it forwards $p$ through that link (i.e., no color change).
\item If the ingoing link is colored $c_i$ and the outgoing link colored $c_i$ has failed, then it forwards $p$ through 
the outgoing link colored $c_{i+1}$. If that link failed, forwards on the outgoing link colored $c_{i+2}$, where each subscript
is modulo $3$.
\end{enumerate}

We now show that this routing scheme is $2$-resilient. 
W.l.o.g, assume that a packet $p$ is first routed along the spanning tree colored $c_0$
(see Fig.~\ref{fig:2-resiliency}).
\begin{figure}[ht]
 \begin{center}
 \includegraphics[width=.6\columnwidth]{figures/2-resiliency.pdf}
 \caption{Proof of Technique 2 of Theorem~\ref{theo:2-resiliency}. Dashed
 colored lines represent paths in the graph. }
 \label{fig:2-resiliency}
 \end{center}
\end{figure}
Either $p$ reaches $d$ or it encounters at a vertex $x$ a failed link $(x,y)$.
In the second case, $p$ is rerouted along a path colored $c_1$. Observe that, either $p$ reaches $d$ 
or it encounters at a vertex $w$, a failed link $(w,z)$.
In the latter case, observe that $w\neq x$, otherwise we have a loop colored $c_1$ that 
contains $x$. Hence, $(x,y)\neq(w,z)$ and no more links can fail. Vertex $w$
reroutes $p$ along a path colored $c_2$. Now, either $p$ reaches $d$ or it encounters at 
a vertex in $u \in \{x,y,w,z\}$, a failed link. In the latter case,
observe that $u\neq x$, since $(x,y)$ is colored $c_0$ from $x$ to $y$ and $u\neq w$, 
since $(w,z)$ is colored $c_1$ from $w$ to $z$. Moreover,
$u\neq z$, otherwise we have a loop colored $c_2$ that contains $(w,z)$. Hence, $u=y$ and 
$u$ reroutes $p$ along $c_0$. Now, observe that either $p$
reaches $d$ or it encounters at $z$ the failed link $(w,z)$. In the latter case, $z$ 
reroutes $p$ on $c_1$. Suppose, by contradiction, 
that $p$ does not reach $d$. It means that it encounters at least a failed link colored 
$c_1$. However, the only outgoing link colored $c_1$ is
$(w,z)$ from $w$ to $z$, which implies that there exists a loop colored $c_1$ that 
contains $(w,z)$, a contradiction.
\end{proof}

\vspace{2mm}
\rephrase{Theorem}{\ref{theo:hypercube-resiliency}}{
 \HypercubeResiliency
}
\vspace{2mm}

We now prove the theorem with the help of several lemmas.

\vspace{.1in}
\noindent
{\bf k-dimensional hypercubes definition. }
A \emph{k-dimensional hypercube} is a graph with $2^k$ vertices where each vertex can 
be labeled with a distinct $k$-digits string of zeros and ones in such a way that two vertices are
adjecent if and only if their labels differ in exactly one coordinate.
Let $L_k$ be the set of all possible string with $k$ digits in $\{0,1\}$. 
Let $L_k^*$ be the set of all possible string with $k$ digits in $\{0,1,*\}$. 
Given a label $l \in L_k$, $l(i)$ denotes the value of the element at coordinate $i$, with $i=1,\dots,k$.
% We say that a label $l \in L_k$ \emph{matches} a label $l^* \in L_k^*$ if for every coordinate $i=1,\dots,k$, we have 
% that $l(i)=l^*(i)$ unless $l^*(i)=*$.
We denote by $H_k$ a  $k$-dimensional hypercube, by $v_l$ the unique vertex in $H_k$ with label $l$.

% and by $S_{l^*}$ the subgraph of $H$ induced by vertices with a label that matches $l^*$, where $l^* \in L_k^*$.

\begin{property}\label{prop:hypercube-construction}
 A $k$-dimentional hypercube can be constructed from two $(k-1)$-dimensional hypercubes by connecting
 vertices with the same label by an edge. Labels are updated by prepending a $0$ $(1)$ at each vertex label
 in the first (second) sub-hypercube.
\end{property}


% \begin{property}\label{prop:hypercube-space} 
%  Subgraph $S_{l^*}$ is a $m$-dimensional hypercube, where $m$ is the number of $*$ in $l^*$. 
% \end{property}

\vspace{.1in}
\noindent
{\bf d-dimensional hypercubes are (d-1)-resilient. }
% We now prove that a $k$-dimensional hypercube is $(k-1)$ resilient. 
% We partition a $H_k$ hypercube in $k$ partitions as follows. Let $l_m^*=(0,\dots,0,1,\dots,1)$ be a string with $m$ zeros
% followed by $k-m$ ones. A partition $H'_m$, with $m \in \{0,1,\dots,k-1,k\}$, of $H_k$ is a subgraph 
% of $H_k$ induced by vertices in $\{d\}$, if $m=k$, or by vertices in $V(S_{l_m^*})\setminus V(S_{l_{m+1}^*})$ otherwise.
% 
We assume, w.l.o.g., that vertex $d$ with label $(0,\dots,0)$ is the destination vertex. 
We construct a connectivity-resilient routing scheme based on $k$ directed arc-disjoint spanning trees $T_1,\dots,T_k$
rooted at $d$.
A set of spanning trees is \emph{arc-disjoint} if for any pair of them, they do not have any directed edge in common.
We use the term \emph{arc} and directed edge interchangeably.
% Let $n_i$, with $i=1,\dots,k$, be the neighbor of $d$ such that $(n_i,d)$ belongs to $T_i$.

% We introduce some notations. 

 We say that a routing scheme is \emph{\nameprop} if the following two properties hold:

\begin{enumerate}[i)]
 \item If a packet must be routed through a spanning tree $T_i$, with $i=1,\dots,k$, but the outgoing link is failed,
 then at least $i$ links failed.
 \item A packet never enter an endless loop. Eventually a vertex detects that at least $k$ links failed.
\end{enumerate}

Intuitively, a \nameprop routing scheme guarantees that a single link failure cannot prevent a packet from being forwarded
on two different spanning trees.

% \begin{enumerate}[i)]
%  \item If a packet is routed through an arc belonging to a spanning tree $T_i$, with $i=1,\dots,k$, then at least $(i-1)$ 
% links failed.
%  \item If $k$ links fail either a packet reaches $d$ or a vertex detects that $k$ links failed while it tries to forward
%  it through $T_k$.
% \end{enumerate}

% \begin{property}\label{lemm:hypercube-k-failures-detection}
%  A \nameprop routing scheme with $k$ arc-disjoint spanning trees is such that either a packet $p$ reaches its destination
%  or a vertex detects that $k$ links failed while it unsuccessfully tries to forward $p$ through $T_k$.
% \end{property}

 \begin{figure}[tb]
  \centering
    \includegraphics[width=.6\columnwidth]{figures/hypercube-embedding-2x2}
    \caption{A $2$-dimensional hypercube with two arc-disjoint spanning trees (solid black and dashed red). }
\label{fig:hypercube-partitioning-base-case}
\end{figure}
% 
\begin{figure}[tb]
  \centering
    \includegraphics[width=\columnwidth]{figures/hypercube-embedding-2x2x2}
    \caption{A $3$-dimensional hypercube with three arc-disjoint spanning trees (solid black, dashed red, and dotted blue). }
\label{fig:hypercube-partitioning-induction}
\end{figure}
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2-red}
%     \caption{A $3$-dimensional hypercube with a red spanning tree.}
% \label{fig:hypercube-partitioning-induction-red}
% \end{figure}
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2-black}
%     \caption{A $3$-dimensional hypercube with a black spanning tree.}
% \label{fig:hypercube-partitioning-induction-black}
% \end{figure}
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2-blue}
%     \caption{A $3$-dimensional hypercube with a blue spanning tree.}
% \label{fig:hypercube-partitioning-induction-blue}
% \end{figure}
% 
\begin{figure}[tb]
  \centering
    \includegraphics[width=\columnwidth]{figures/hypercube-embedding-2x2x2x2}
    \caption{A $4$-dimensional hypercube with four arc-disjoint spanning trees (solid black, dashed red, dotted blue, and dash dotted green). }
\label{fig:hypercube-partitioning-induction-16}
\end{figure}
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2x2-red}
%     \caption{A $3$-dimensional hypercube with a red spanning tree.}
% \label{fig:hypercube-partitioning-induction-red-16}
% \end{figure}
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2x2-black}
%     \caption{A $3$-dimensional hypercube with a black spanning tree.}
% \label{fig:hypercube-partitioning-induction-black-16}
% \end{figure}
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2x2-blue}
%     \caption{A $3$-dimensional hypercube with a blue spanning tree.}
% \label{fig:hypercube-partitioning-induction-blue-16}
% \end{figure}
% % 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2x2x2x2-green}
%     \caption{A $3$-dimensional hypercube with a green spanning tree.}
% \label{fig:hypercube-partitioning-induction-green-16}
% \end{figure}
% % 
% 
% \begin{figure}[tb]
%   \centering
%     \includegraphics[width=.7\columnwidth]{figures/hypercube-embedding-2}
%     \caption{A $6$-dimensional hypercube. Vertices are labeled with $(l_1, l_2, l_3, l_4, l_5,l_6)$.
%     Destination vertex $d$ has label $(0,0,0,0,0,0)$ and its neighbors are shown with bolded circles connected through an edge
%     to $d$. }
% \label{fig:hypercube-partitioning}
% \end{figure}
% 

 We construct our \nameprop routing scheme recursively on the size of the hypercube $H_k$.
 If $k=2$, i.e., four vertices connected through a cycle, the statement trivially holds. Routing is as follows 
 (see Fig.~\ref{fig:hypercube-partitioning-base-case}).
 A vertex first tries to route a packet counterclockwise (i.e., through the red spanning tree). When a vertex receives a packet 
 from one of its neighbors, it does not change its direction, unless the outgoing link failed. 
 It is easy to verify that this routing scheme is \nameprop. In fact, a packet is not routed on the red spanning tree
 only if at least one link failed. If a packet $p$ cannot reach its destination through the balck spanning tree, then 
 at least two links failed and the vertex that is not able to forward $p$ on the black tree can detect it.

 We now show how to construct a \nameprop routing scheme $R_k$ for a $k$-dimensional hypercube $H_k$, based on a 
 \nameprop routing scheme $R_{k-1}$ for a $(k-1)$-dimensional hypercube $H_{k-1}$. 
 By Property~\ref{prop:hypercube-construction}, we can construct $H_k$ based on two copies $H_A$ and $H_B$ of $H_{k-1}$, where 
 $H_{k-1}^A=S_{(0,*,\dots,*)}$ and $H_{k-1}^B=S_{(1,*,\dots,*)}$ .
%  (see Fig.~\ref{fig:hypercube-partitioning-induction}
%  or Fig.~\ref{fig:hypercube-partitioning-induction-16}).
 Both $H_{k-1}^A$ and $H_{k-1}^B$ are $(k-1)$-dimensional hypercubes. Let $l_{d_A}=(0,\dots,0)$ and $l_{d_B}=(1,0,\dots,0)$
 be destination vertices for $H_{k-1}^A$ and $H_{k-1}^B$, respectively. 
%  
%  Since $R$ is \nameprop, 
%  
%  if a packet must be routed through a spanning tree $T_i$, with $i=1,\dots,k$, but the outgoing link is failed,
%  then at least $i$ links failed.
%  
%  there exists a routing scheme
%  for both $H_A$ and $H_B$ such that both propeperties (i) and (ii) hold, where we assume that vertices $d_A$ and $d_B$,
%  with $l_{d_A}=(0,\dots,0)$ and $l_{d_B}=(1,0,\dots,0)$, are destination vertices for $H_A$ and $H_B$,
%  respectively. 
%  Moreover, either a packet reaches $d_A$ ($d_B$) or a vertex detects that more than $(k-2)$ 
%  links failed in $H_A$ ($H_B$). 
%  
%  We now define a routing scheme such that (i) and (ii) hold for $H_k$. 
%  Intuitively, we try to route in each hypercube as long as less than $k-1$ links fail or we reach a neighbor
%  of the destination vertex. In that case, 
%  a packet is rerouted to the other hypercube, where it is guaranteed to do not encounter any other link failure.
%  If a packet $p$ is originated in $H_B$, we try to send it to $H_A$. If we fail, $p$ is routed in $H_B$ 
%  towards $d_B$, where it is guaranteed to reach $d$ via a direct link. 
%  
%  We now describe our routing scheme construction in detail. 
 We use routing scheme $R_{k-1}$ to route packets within $H_{k-1}^A$ and $H_{k-1}^B$ to destinations $d_A$ and $d_B$, respectively. 
 The reader can refer to Fig.~\ref{fig:hypercube-partitioning-induction-16}, where a $4$-dimensional hypercube
 $H_4$ is built based on a \nameprop routing scheme shown in Fig.~\ref{fig:hypercube-partitioning-induction} for a 
 $3$-dimensional hypercube $H_3$.
 Let $T_1^A,\dots,T_{k-1}^A$ and $T_1^B,\dots,T_{k-1}^B$ be the $(k-1)$ arc-disjoint spanning trees used in $H_{k-1}^A$ and $H_{k-1}^B$
 to route packets, respectively. We construct $k$ arc-disjoint spanning trees $T_1,\dots,T_k$ for $H_k$ as follows.
%  Let $n_i$, with $i=1,\dots,k$, be the neighbor of $d$ such that $(n_i,d)$ belongs to $T_i$.
 Let $n_i^A$ ($n_i^B$) be the unique neighbor of $d_A$ ($d_B$) such that arc $(n_i^A,d_A)$ ($(n_i^B,d_B)$) belongs to $T_i^A$ ($T_i^B$).
 For each $i=1,\dots,k-2$, let $T_i$ be the union of both $T_i^A$ and $T_i^B$  plus arc $(n_i^B,n_i^A)$.
 Moreover, for each $i=1,\dots,k-2$, we reverse arc $(n_i^B,d_B)$ in $T_i^B$.
%  (see Fig.~\ref{fig:hypercube-partitioning-induction-red-16}
%  and Fig.~\ref{fig:hypercube-partitioning-induction-black-16}).
 Tree $T_k$ is constructed from $T_{k-1}^B$ 
 by adding all the edges from $H_{k-1}^A$ to $H_{k-1}^B$ and reversing arc $(d_A,d_B)$. 
%  In the example in Fig.~\ref{fig:hypercube-partitioning-induction-16}),
%  $T_4$ is constructed based on the blue spanning tree of Fig.~\ref{fig:hypercube-partitioning-induction}.
 Tree $T_{k-1}$ is constructed from $T_{k-1}^A$ 
 by adding all the arcs from $H_{k-1}^B$ to $H_{k-1}^A$ that do not belong to any $T_1,\dots,T_{k-2},T_k$.
 Moreover, we add into $T_{k-1}$ arc $(d_B,n_{k-1}^B)$ and all arcs $(n_i^B,d_B)$, with $i=1,\dots,k-2$.
 In the example of Fig.~\ref{fig:hypercube-partitioning-induction-16},
 both $T_3$ and $T_4$ are constructed based on the blue spanning tree of Fig.~\ref{fig:hypercube-partitioning-induction}.
 
%  Routing is as follows. A packet is first routed thorugh $T_1$. A packet is routed along the next spanning tree only
%  if it cannot be forwarded through the same spanning tree. 

 Intuitively, our routing scheme construction works as follows. A packet is first routed through $T_1$. 
 A vertex reroutes a packet from $T_i$ to $T_{j}$, with $1\le i<j\le k-1$, only if it cannot be forwarded through any 
 $T_i,\dots,T_{j-1}$. A vertex $v$ reroutes a packet $p$ from $T_i$ to $T_1$, with $1< i\le k$, only if it receives $p$
 from a vertex whose label can be obtained from $v$'s label by switching one $0$ with a $1$. 
 Several exceptions apply to the last rule. Namely, if a packet is sent from a vertex $v_{(*,\dots,*,1,0,\dots,0)}$ to
 a vertex $v_{(*,\dots,*,0,\dots,0)}$, where the number of '*' is the same for both vertices, we do not switch our routing tree.
 For example, in Fig.~\ref{fig:hypercube-partitioning-base-case}, we do not switch back to the red spanning tree when
 a packet is routed from $v_{(1,1)}$ to $v_{(1,0)}$.  In Fig.~\ref{fig:hypercube-partitioning-induction-16}, we do not switch
 from the green spanning tree to the red one neither when a packet is routed from $v_{(1,1,0,0)}$ to $v_{(1,0,0,0)}$ nor when 
 a packet is routed from $v_{(1,1,1,0)}$ to $v_{(1,1,0,0)}$. We show in Fig.~\ref{fig:hypercube-partitioning-induction-16-rerouting}
 all the arcs that are incident to vertices that reroute packets received from these arcs through the red spanning tree.
 Observe that there are no green arcs depicted, which is a property that we prove in the following lemma.

\begin{figure}[tb]
  \centering
    \includegraphics[width=\columnwidth]{figures/hypercube-embedding-2x2x2x2-no-rerouting}
    \caption{A $4$-dimensional hypercube where only arcs that perform rerouting operations are depicted.}
\label{fig:hypercube-partitioning-induction-16-rerouting}
\end{figure}

\begin{lemma}\label{lemm:hypercube-t-k}
 When a packet is routed through $T_k$, it is never rerouted through any other spanning tree.
\end{lemma}
\begin{proof}
 We prove it by induction on $k$. In the base case $k=2$, it is easy to see that when a packet is sent on the black spanning
 tree, then it is routed along $v_{(0,1)},v_{(1,1)},v_{(1,0)},v_{(0,0)}$, and a vertex is never allowed to reroute a packet
 on the red spanning tree.
 In the inductive step $k>2$, observe that $T_k$ by inductive hypothesis, the statement holds for every arc in $H_{k-1}^B$.
 Moreover, every other arc is either oriented from $H_{k-1}^A$ to $H_{k-1}^B$, which means that the first coordinated is 
 switched from $0$ to $1$, or it is oriented from $v_{(1,0,\dots,0)}$ to $v_{(0,\dots,0)}$, which means that it is not rerouted
 through any other spanning tree. 
\end{proof}


 \begin{lemma}
  $R_k$ is a \nameprop routing scheme.
 \end{lemma}
 \begin{proof}
  Consider a packet $p$ that is originated in $H_{k-1}^A$. Observe that all the arcs from $H_{k-1}^A$ to
  $H_{k-1}^B$ belong to $T_k$. Hence, since routing in $H_{k-1}^A$ is \nameprop w.r.t. the first $k-1$ spanning trees, 
  a vertex detects if $k-1$ link failures prevent $p$ from reaching $d_A$.
  In that case, a packet is forwarded through $T_k$ and it is routed entirely within $H_{k-1}^B$ and a single edge between
  $H_{k-1}^A$ and $H_{k-1}^B$. By 
  Lemma~\ref{lemm:hypercube-t-k}, $p$ is not rerouted to any other spanning tree. Hence, either $p$ reaches $d_B$ and, in turn, $d_A$ 
  or a link in $H_{k-1}^B$ or between $H_{k-1}^A$ and $H_{k-1}^B$ must have failed. 
  This link is different from  any other of the $(k-1)$ links that failed in $H_{k-1}^A$, which leads to a total
  of $k$ link failures. The vertex that cannot forward through $T_k$ detects that at least $k$ links failed. 
  Hence, in this case, our routing scheme is \nameprop since a packet will never enter a loop without any vertex detecting
  that $k$ links failed.
  
%   Then, by induction hypothesis, $p$ either reaches $d_a$ or
%   a vertex $v$ detects that at least $k-1$ links failed while it tries to forward it through $T_{k-1}$. In that case, 
%   $p$ is forwarded through $T_k$, which, by construction, let $p$ reach $H_B$. Observe that if $p$ cannot be forwarded 
%   through $T_k$ to $d$, it means that a link failed in $H_B$ or link $(d_B,d_A)$ failed.  Hence, the vertex that is unable to forward $p$ through 
%   $T_k$ detects that at least $k$ links failed.
  
  We now consider a packet $p$ that is originated in $H_{k-1}^B$. Observe that since the routing scheme
  within $H_{k-1}^B$ is partly different from $R_{k-1}$, we first need to analyze these differences. 
  Since our changes in the routing scheme only involve neighbors of $d_B$ and $T_{k-1}$, we have that, if a 
  packet $p$ is routed through $T_i$, with $i=1,\dots,k-2$, we are guaranteed that if $p$ reaches $n_i^B$, 
  it is either routed to a vertex $a$ in $H_{k-1}^A$ or link $(n_i^B,a)$ failed. If the link failed, $n_i^B$ behaves 
  exactly as link $(n_i^B,d_B)$
  failed in $R_{k-1}$. That is, it forwards $p$ through $T_{i+1}$ in $H_{k-1}^B$ and routing is still \nameprop
  because identical to $R_{k-1}$. 
  Hence, we have that if $p$ is routed to a vertex in $H_{k-1}^A$ through a spanning tree $T_i$, with $i=1,\dots,k-1$, then 
  at least $i-1$ links failed between $H_{k-1}^B$ and $H_{k-1}^A$ or in $H_{k-1}^B$. 
  Observe that when a packet is routed from a vertex in 
  $H_{k-1}^B$ to a vertex in $H_{k-1}^A$ through a spanning tree $T_i$, with $i=1,\dots,k-2$, it is rerouted 
  to $T_1$ in $H_{k-1}^A$ and we already proved our scheme is \nameprop for packets that are originated in $H_{k-1}^A$. 
  
%   unless $i=1$. If a packet $p$ is routed from a vertex in 
%   $H_{k-1}^B$ to a vertex in $H_{k-1}^A$, then, by inductive hypothesis,
%   if $p$ cannot reach $d_a$ and it cannot be forwarded through $T_{k-1}$, then $k-1$ links failed in $H_{k-1}^A$. In that case, by
%   construction of our routing scheme, $p$
%   is rerouted through $T_k$ to a vertex in $H_{k-1}^B$, where it is either routed to $d_B$ within $H_B$ and then
%   to $d_A$, or it is blocked by a failed link, which must be a different link from the $k-1$ links that failed in $H_{k-1}^A$. 
%   Hence, if $p$ cannot be routed through $T_k$, at least $k$ links failed, which proves the statement in this case.
  
% through $T_{i}$, 
%   with $i=1,\dots,k-1$, in $H_B$ only if at least $(i-1)$ links failed between $H_B$ and $H_A$ or in $H_B$. 
  We now consider routing through $T_{k-1}$ in $H_{k-1}^B$ (i.e., 
  the blue spanning tree in Fig.~\ref{fig:hypercube-partitioning-induction-16}) and $T_k$. Three cases are possible: (i)
  $p$ is located at $d_B$, (ii) $p$ is located at any vertex $n_1^B,\dots,n_{k-2}^B$, or (iii) $p$ is located 
  at any other vertex. 
%   
  In case (i), either $(d_B,d_A)$ failed or not. In the latter case, $p$ reaches its destination,
  otherwise $(k-1)$ links failed and $p$ is sent , if possible, to $n_{k-1}^B$, where it is either forwarded to $H_{k-1}^A$ or, in case
  of another link failure, rerouted through $T_k$ to $d_B$. Then, if link $(d_B,d_A)$ failed, we have that at least $k$ links failed and
  vertex $d_B$ can detect it.
%   
  In case (ii), either $(n_{i}^B,d_b)$ failed or not. In the latter case, 
  $p$ is sent to $d_B$ and we are in case (i). Otherwise, otherwise $(k-1)$ links failed 
  and $p$ can be sent through $T_k$. Observe that, by construction, $T_k$ equals $T_{k-1}^B$ in $H_{k-1}^B$.
  Hence, this corresponds to route according to $R_{k-1}$, which
  guarantees that if $p$ cannot be send through $T_k$, then at least $k$ links failed.
%   
  In case (iii),  $p$ is sent to $H_{k-1}^A$ unless the outgoing link failed. In that case, $k-1$ links failed and $p$ is forwarded
  through $T_k$. By 
  Lemma~\ref{lemm:hypercube-t-k}, $p$ is not rerouted to any other spanning tree. Hence, as in the previous case, this 
  corresponds to route according to $R_{k-1}$, which guarantees that if $p$ cannot be send through $T_k$, then at least $k$ links failed.
  This concludes the proof of this theorem.
 \end{proof}

 The following corollary easily follows by the previous lemma and proves Theorem~\ref{theo:hypercube-resiliency}.
 
\begin{corollary}
 $R_k$ is $(d-1)$-resilient.
\end{corollary}

 \noindent\textbf{More results on hypercubes. } The longest path of a spaning tree is $O(\lg{n})$, where $n$ is the number of vertices
 in the spanning tree. This is much better than technique that uses hamiltonian cycles, where the longest path is $O(n)$.
 \textbf{Open problem:} What is the maximum strech?




\vspace{2mm}
\rephrase{Theorem}{\ref{theo:generalized-hypercube-resiliency}}{
 \GeneralizedHypercubeResiliency
}
\vspace{2mm}

\begin{proof}
 \notemarco{TODO}.
\end{proof}

\vspace{.1in}
\noindent\textbf{Hamiltonian-Based Routing Schemes}
The following technique can be used to obtained resilient routing
in specific cases. If a graph contains $k$ hamiltoninan cycles, i.e. an
\emph{hamiltonian cycle} is a cycle that visits all vertices exactly once,
then we can use this cycles to sustain $2k-1$ link failures.
Routing is as following. Each cycle is 
directed in some way and all cycles are ordered in a sequence. Packet starts to 
traverse the first cycle according to its orientation. 
If a packet encounters a failed link while it is sent 
according to the orientation of the cycle, it is sent backwards
along the same cycle. If 
the packet encounters a failed link while it is forwarded
backward through a cycle,
it is sent through the next cycle in the sequence with the correct cycle orientation. 
Note that each 
vertex has at least two links that belong to a different hamiltonian cycles. 
Therefore it is always 
possible to switch from one cycle to the other one. Because 
cycles are edge-independent, a packet will never 
encounter the same failed link twice. Therefore 
for any $2k-1$ failed links any packet will be 
guided to the destination using proposed routing 
scheme.
\footnote{This technique could be used to find $(2d-1)$-resilient routing
for $2d$-dimensional hypercubes, which are guaranteed to have $d$ disjoint hamiltonian cycles~\cite{}. 
However, this technique has a drawback. Consider a neighbor vertex of $d$. If the direct link to $d$ is failed,
it must route a packet in the opposite direction, which means that this packet will visit all the vertices of
the graph before eventually reach the destination. In our previous construction, we expect to have much smaller
strech factors. }

We use this technique to achieve $3$-resiliency on $4$-connected grid graphs.

\vspace{2mm}
\rephrase{Theorem}{\ref{theo:grid-resiliency}}{
 \GridResiliency
}
\vspace{2mm}

\begin{proof}
We present a $3$-resilient 
routing scheme for grid graphs. We consider 
a rectangular grid with additional links wrapped 
around borders (see Fig.~\ref{fig:grid1}). This 
is a $4$-connected graph.

Our routing scheme relies on graph 
decomposition to $2$ edge-independent 
Hamiltonian cycles. We prove that such decomposition always 
exists. We provide patterns for different 
parity of grid dimensions which are extendible 
by adding two rows or columns for such 
decomposition. Fig.~\ref{fig:grid1}, Fig.~\ref{fig:grid2}, and Fig.~\ref{fig:grid3} shows all 
possible parity cases. Two cycles are marked 
with different line types. Repeatable blocks 
are highlighted with curve brackets.


% \begin{figure*}[p]
% %\vspace{-1in} 
% \centering
% \begin{subfigure}[t]{1in}
% \centering
% % \includegraphics[width=1in, height=1in]{figures/grid-oo.pdf}
% \caption{Odd-Odd}
% \label{fig:grid1}
% \end{subfigure}%
% \qquad
% \begin{subfigure}[t]{1in}
% \centering
% \includegraphics[width=1in, height=1in]{figures/grid-ee.pdf}
% \caption{Even-Even}
% \label{fig:grid2}
% \end{subfigure}%
% \qquad
% \begin{subfigure}[t]{1in}
% \centering
% \includegraphics[width=1in, height=1in]{figures/grid-eo.pdf}
% \caption{Even-Odd}
% \label{fig:grid3}
% \end{subfigure}%
% \caption{Grid decomposition patterns to $2$ Hamiltonian cycles for Odd-Odd, Even-Even and Even-Odd grid graphs}
% \label{fig:grid}
% \end{figure*}
% 


\begin{figure}[t]
% \centering
\begin{minipage}[t]{0.3\columnwidth}%
% \vspace{0.3in}
\includegraphics[width=\columnwidth]{figures/grid-oo.pdf}
\caption{Odd-Odd case.}\label{fig:grid1}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.3\columnwidth}%
\includegraphics[width=\columnwidth]{figures/grid-ee.pdf}
\caption{Even-Even case.}\label{fig:grid2}
\end{minipage}
\hfill
\begin{minipage}[t]{0.3\columnwidth}%
% \vspace{0.3in}
\includegraphics[width=\columnwidth]{figures/grid-eo.pdf}
\caption{Even-Odd case}\label{fig:grid3}
\end{minipage}%
\end{figure}
\end{proof}

\noindent\textbf{More results. }Using connectivity-resiliency routing scheme for grid topologies described in the next paragraph we can prove that
 the same result holds also for grid-hypercubes. The proof is similar to the generalized hypercube.



\vspace{2mm}
\rephrase{Theorem}{\ref{theo:clos-resiliency}}{
 \ClosResiliency
}
\vspace{2mm}

\begin{proof}
 TODO
\end{proof}

We now prove the following theorem.

\vspace{2mm}
\rephrase{Theorem}{\ref{theo:chordal-resiliency}}{
 \ChordalResiliency
}
\vspace{2mm}

We consider the vertex-connected case and vertex failures instead of 
link failures. We should be able to prove it also for standard link-connectivity and
link failures. 

We consider a problem where the input graph is chordal, i.e., it does
not contain any induced cycle of length $4$ or more. 
% The more general result
% for graphs that do not have chordless induced cycles of length $5$ or more
% does not depend on this section, so the reader can eventually directly skip to 
% Theorem~\ref{theo:c5free-resiliency}.

\vspace{.1in}
\noindent
{\bf k-connected chordal graphs are (k-1)-resilient. }
A graph is {\em chordal} if it does not have an induced cycle of length $4$ or more.
The following result is known for chordal graphs. A {\em vertex separator} $S$ of a graph $G$ is
a set of vertices, such that after their removal from $G$, $G$ has at least two components.
A vertex separator is minimal, if it is the vertex separator of smallest cardinality.


\begin{lemma}\label{lemm:induced-transitive-property}
 Let $G$ be a graph that does not contain an induced subgraph $G'$. Then,
 any induced subgraph of $G$ does not contain an induced subgraph $G'$.
\end{lemma}
\begin{proof}
 Consider a graph $G$ that does not contain an induced subgraph $G'$ and  consider
 an arbitrary induced subgraph $G[V']$ of $G$, with $V'\subseteq V(G)$.
 Suppose, by contradiction, that  $G'$ is an induced subgraph of $G[V']$ induced by a set of 
 vertices $V''$. Then, $G[V'']$ is also equal to $G'$, which is a contradiction 
 since $G$ does not contain $G'$ as an induced subgraph.
\end{proof}

\begin{corollary}\label{coro:induced-transitive-property-chordal}
 Any induced subgraph of a chordal graph is a chordal graph.
\end{corollary}

% \begin{corollary}\label{coro:induced-transitive-property-negc5}
%  Any induced subgraph of a \cfivefree graph is a \cfivefree graph.
% \end{corollary}
% \begin{proof}
%  Because of Lemma~\ref{lemm:induced-transitive-property}.
% \end{proof}


\begin{lemma}\label{lemm:chordal-graph-induced-property}
 Let $G$ be a $k$-vertex-connected chordal graph and $S$ be a minimal vertex separator of $G$.
 Let $A_1, \dots, A_n$ be the $n$ set of vertices belonging to the $n$ disconnected components 
 of $G$ after the removal of vertices in $S$ from $G$.
 Each $G[A_i \cup S]$, with $i \in [n]$, is a $k$-vertex-connected graph.
\end{lemma}
\begin{proof}
 We prove
 that the vertex-connectivity is preserved. Consider any subgraph $G[A_i \cup S]$, with $i \in [n]$. 
 Consider any two vertices $v$ and $z$ in  $A_i \cup S$. Two cases are possible: either
 both $v$ and $z$ are in $S$ or at least one betweem $v$ and $z$ is not in $S$.
 
 In the first case (both $v$ and $z$ are in $S$), If the graph $G[S]$ has at least $k+1$ vertices, it is 
   well-known\cite{} that a minimal vertex separator $S$ of a 
   chordal graph is a clique. Hence, $G[S]$ is $k$-connected in this case.
   Otherwise, if $S$ has exactly $k$ vertices (it cannot have less than $k$ vertices 
   otherwise $G$ is not $k$-connected), then each vertex from $S$ must be connected 
   to some node in a certain $A_i$, with $i \in [n]$, (otherwise we could 
   exclude some nodes from $S$ and it will still be a separator). Therefore, there exists 
   at least one path in $A_i$, connecting $v$ and $z$. And there are $k-1$ vertex disjoint paths in $S$.
   This proves that vertices in $S$ are $k$-vertex-connected each other.
   
 In the second case (i.e., at least one between $v$ and $z$ is not in $S$), w.l.o.g, we assume
  that $z$ is not is $S$. Let $p_1,\dots,p_k$ be the $k$-vertex-disjoint paths between $v$ and $z$.
  Consider any path $p_j$, with $j \in [k]$. If $p_j$ only traverses vertices in $V(G[A_i \cup S])$, then this path also 
  exists in $G[A_i \cup S]$. Otherwise, if $p_j$ traverses vertices not in $A_i$, then it must cross $S$. 
  It is well-known
  that each minimal vertex separator of a chordal graph is a complete graph, i.e., each pair of vertices
  in the minimal vertex separator are adjacent each other. Let $s_v$ ($s_z$) be the closest vertex to $v$ ($z$)
  on $p_j$. We replace the subpath of $p_j$ between $s_v$ and $s_z$ with a single edge 
  $(s_v,s_z)$. Hence, each path $p_j$ is either contained in $G[A_i \cup S]$ or it is 
  replaced by a path in $G[A_i \cup S]$.
\end{proof}


\begin{theorem}\label{theo:chordal-graphs-resiliency}
 A $k$-vertex-connected chordal graph is $(k-1)$-vertex-resilient.
\end{theorem}
\begin{proof}
 Let $G$ be a $k$-connected chordal graph.
 We prove by induction on the size of $G$ that there exists a routing scheme
 such that, given any vertex $v$ of $G$ and a destination $d$ of $G$, $v$ can reach $d$
 under at most $k-1$ link failures.
 In the base case, $G$ is a clique. We show a routing scheme that is $k-1$ resilient
 for a clique. $G$ consists of a destination vertex $d$ and $k$ different vertices $v_1$,\dots,$v_k$.
 Let $f^{v_i}$ be a circular ordering such that $v_i$ forwards a packet received from $v_l$
 to the first vertex that succeeds $v_l$ for which $v_i$ has an available outgoing link.
 We can prove that this is $k-1$ resilient \notemarco{to be proved, easy}.
 In the inductive step, consider a minimal\footnote{a minimal 
 vertex separator is not necessarily a minimum vertex separator.} vertex separator 
 $S$ of $G$. $S$ has cardinality at least $k$,
 otherwise $G$ would not be $k$-vertex-connected. After the removal of $S$ from $G$, 
 $G$ has $n$ components, with $n\ge2$. We denote by $A_1$, \dots, $A_n$ the set of vertices
 in each of these disconnected components. Observe that,
 by Lemma~\ref{lemm:chordal-graph-induced-property} and Corollary~\ref{coro:induced-transitive-property-chordal}, 
 each graph $G[A_i \cup S]$ is a $k$-vertex-connected chordal graph.
 W.l.o.g., assume that $d$ is contained in $A_1 \cup S$. 
 By induction hypothesis, each vertex of $A_1 \cup S$ can reach $d$ under $k-1$ failure. 
 For each vertex $v$ in a component $A_i$, $i> 1$, by induction hypothesis, $v$ can reach
 a vertex $s \in S$ under $k-1$ failures. Then, $s$ can use the routing scheme computed for $G[A_1 \cup S]$ 
 in order to reach $d$ under $k-1$ vertex failures, which proves the theorem.
\end{proof}







